Influence Functions for Sequence Tagging Models

Many language tasks (e.g., Named Entity Recognition, Part-of-Speech tagging, and Semantic Role Labeling) are naturally framed as sequence tagging problems. However, there has been comparatively little work on interpretability methods for sequence tagging models. In this paper, we extend influence functions - which aim to trace predictions back to the training points that informed them - to sequence tagging tasks. We define the influence of a training instance segment as the effect that perturbing the labels within this segment has on a test segment level prediction. We provide an efficient approximation to compute this, and show that it tracks with the true segment influence, measured empirically. We show the practical utility of segment influence by using the method to identify systematic annotation errors in two named entity recognition corpora. Code to reproduce our results is available at https://github.com/successar/Segment_Influence_Functions.

==> gaz_extra.tex <==
% \subsection{Gazetter labeled CoNLL}

% \newcommand{\M}[1]{$\mathcal{#1}$}
% \newcommand{\B}[1]{$\mathbf{\mathbb{#1}}$}

% We divide CoNLL training set in two parts -- An \emph{expert} labeled set \M{E} of size 500 examples and a pool set \M{P} of remaining examples which (we \emph{assume}) we don't know the true labels of. The goal is to generate the best possible \emph{constructed} set \M{C} out of \M{P} by adding labels to examples in \M{P}. Note \M{C} can either contain all \M{P} examples labeled or only a subset of those (that is \M{C} $\subseteq$ \M{P}).

% We measure best possible in terms of performance on CoNLL validation set. And since we do know the true labels of set \M{P}, we measure precision, recall and F1 score of \M{C} with respect to true labels of \M{P}.

% \noindent\paragraph{Gazetteer Labeling Procedure}
% We use a gazetteer derived from wikidata corpus, where each string is matched to a subset of \{PER, ORG, LOC\} labels. 
% For each example in \M{P}, we identify all tokens consisting with PROPN part-of-speech tag (using SpaCy). For each segment of PROPN tokens (that is consecutive tokens all with PROPN tag), we identify for all possible spans whether they appear in lookup table and get its \emph{label set}. Finally, if two spans have overlapping tokens, we keep the larger one. Applying this procedure to all PROPN segments, we obtain a non-nested set of spans for this example, each span associated with a label set. For example, a sentence like \textsf{Liverpool and Manchester had a match in London.} may get labeled as \textsf{Liverpool/[LOC,ORG] and Manchester/[LOC,ORG] had a match in London/[LOC,ORG].}

% After this processing, gazetteer identified ~23K entities in the pool set. The pool set contains 20K true entities out of which 14K are labeled correctly by the gazetteer (with both span correct and type in the label set). ~800 entities has correct span but don't contain the correct label in the label set, ~2400 entities are partially matched and ~1800 entities are missed entirely. Therefore, approximately 78\% of entities have an exact span while 91\% entities have atleast a partial match. In addition, 14\% of spans identified by the gazetteer are spurious (i.e do not overlap with any true entity) that is 14\% out of the 23K.

% \begin{table*}[htbp!]
%     \centering
%     \begin{tabular}{l|c|c|c}
%          & \multicolumn{2}{c|}{Validation Set} & \\
%         Method to get \M{C} & Trained on \M{C + E} & Trained on \M{C} & True Labels of \M{P}\\\hline
%         \M{P} with True Labels & 0.922 & 0.921 & 1.000 \\
%         \B{E} Prediction on \M{P} & 0.679 & 0.681 & 0.658 \\\hline
%         Oracle Choice & 0.762 & 0.760 & 0.738 \\
%         Random Choice & 0.607 & 0.563 & 0.467 \\
%         Best Label Ordered & 0.504 & 0.502 & 0.518 \\\hline
%         Instance Influence & 0.635 & 0.606 & 0.545 \\
%         Instance Influence + Post Filtering & 0.634 & 0.646 & --- \\
%         Entity Influence & 0.638 & 0.621 & 0.582 \\
%         Entity Influence + Post Filtering & 0.642 & 0.647 & --- \\
%     \end{tabular}
%     \caption{Performance on CoNLL Validation Set and True labels of Pool Set in terms of macro avg F1 score. This is for 100 expert set examples}
%     \label{tab:gaz_conll}
% \end{table*}

% \noindent\paragraph{Variant creation} Our models can only be trained on spans annotated with labels rather than label set. Therefore, we need to collapse these label sets to a single label for each span. Three possible methods exist:

% \begin{enumerate}
%     \item \textbf{All Combinations:} We take all possible combinations of labels for an example. This will create, for example, 8 \emph{\textbf{variants}} in above example.
    
%     \item \textbf{Label Consistent:} For all spans in an example, we choose their labels from corresponding label set set according to same ordering. So for above example, we get two label consistent \emph{variants} -- one where choose LOC for every entity and other where we choose ORG for every entity (\textsf{Liverpool/LOC and Manchester/LOC had a match in London/LOC.} and \textsf{Liverpool/ORG and Manchester/ORG had a match in London/ORG.})
    
%     \item \textbf{Sampling:} For every span, we randomly choose one of the labels from its label set. We repeat this process K times to get K samples (hopefully unique). Here I use K=6 yielding on average 2.22 variants per instance.
% \end{enumerate}

% At the end of this step, we have a set of data \M{PV} containing labeled instances of \M{P} where each example can be associated with multiple overall label sequences (aka variants derived from gazetteer labeling followed by variants creation).

% \noindent\paragraph{Model Training and \M{C} Creation}

% We now train two models - a model \B{E} trained on only the expert set \M{E}, a model \B{PV} trained on the set \M{PV} and a model \B{PVE} trained on \M{PV+E}. While \B{E} is trained using standard CRF training, to train \B{PV} and \B{PVE}, we marginalize over all variants for instances belonging to \M{PV}  -- that is for a given instance $(X, \{Y_1, ..., Y_v\})$ that has $v$ variants, we use the loss

% \begin{equation}
%     L(X, \{Y_1, ..., Y_v\}) = -\log \sum_{i=1}^v P(Y_i | X)
% \end{equation}

% Given these models, we can now construct our \M{C} in a variety of ways. Some baselines are as follows:

% \begin{enumerate}
%     \item \textbf{\B{E} Prediction:} Use \B{E} to predict labels for \M{P} 
%     \item \textbf{\B{PV} Prediction:} Use \B{PV} to predict labels for \M{P} 
%     \item \textbf{Oracle Choice:} For each span in an example identified via gazetteer after gazetteer labeling procedure, identify the best label for it from the associated label set by using the true labels of that example. Note, this oracle only applies to spans identified by gazetteer. This is the best we can hope to achieve after variant filtering methods described below.
%     \item \textbf{Random Choice:} Select a random variant for each instance in \M{P}
%     \item \textbf{Label Consistent Choice:} Select the best label precedence order to be applied across all instances in M{P}. Best will be measured in terms of performance on our held out set.
% \end{enumerate}

% Next we have two methods which use influence to identify best variant for each instance in \M{P}.

% \begin{enumerate}
%     \item \textbf{Instance Influence:} For each variant of an example, we compute the influence with respect to the expert set examples using model \B{E} \note{[note: discuss in meeting why we used \B{E} instead of \B{PV}]}. A variant is assigned a score indicating different between influence on top 5 opposing example and top 5 supporting examples. A high value of this score indicates that a variant opposes expert set \emph{more than} it supports it. As such, we want to keep the variant associated with lowest score here.
%     \item \textbf{Entity Influence:} For every span identified by the gazetteer, we find its entity level influence score across all variants and keep its type from the one with lowest score. So in this case, the final label sequence for a given instance may be composed out of multiple variants. 
    
%     As an example, consider the two variants as 1) \textsf{Liverpool/LOC and Manchester/LOC had a match in London/LOC.} and 2) \textsf{Liverpool/ORG and Manchester/ORG had a match in London/ORG.}. The spans \textsf{Liverpool} and \textsf{Manchester} has lowest entity influence score in second variant and therefore we keep ORG as the label for both. On the other hand, the span \textsf{London} have lower entity influence score in the first variant compared to second, so in this case, we keep the label LOC for it. At the end, the label sequence we get is \textsf{Liverpool/ORG and Manchester/ORG had a match in London/LOC.} even though we did not had it as a variant a priori (assuming we used label consistent method of variant creation).
    
%     \note{[TODO: convert this process to algorithm format. May need a bit more explanation.]}
    
%     \item \textbf{Entity Influence + Post Filtering:} In this case, we take the constructed set using Entity Influence and then filter from it those examples whose Instance Influence score is greater than 0.25. This basically allows us to remove examples that are still bad even after Entity Influence step. This and the following are the only cases where we have that \M{C} $\subseteq$ \M{P}. 
    
%     \item \textbf{Instance Influence + Post Filtering:} In this case, we take the constructed set using Instance Influence and then filter from it those examples whose Instance Influence score is greater than 0.25.  
% \end{enumerate}

% \noindent\paragraph{Results}

% First we present results on the validation set performance in Table~\ref{tab:gaz_conll} when trained on various \M{C} constructions as described above.

% \begin{table*}[htbp!]
%     \centering
%     \begin{tabular}{l|cc|cc}
%         Model &  \multicolumn{2}{c|}{Drug} & \multicolumn{2}{c}{Therapy}\\
%         & Precision & Recall & Precision & Recall \\\hline
%         Expert Only Model & 0.71 & 0.56 & 0.68 & 0.16 \\
%         True train set Model & 0.64 & 0.75 & 0.64 & 0.62 \\
%         RxNorm labeled train set &  0.76 & 0.40 & 0.48 & 0.01 \\
%         RxNorm+MeSH labeled train set &  0.69 & 0.41 & 0.45 & 0.05 \\
%     \end{tabular}
%     \caption{Results of Models trained with Gazetteer for EBM-NLP. We measure performance in terms of token level P/R for Intervention label.}
%     \label{tab:ebm_gaz}
% \end{table*}

% \subsection{EBM NLP Gazetteer Analysis}

% \noindent\paragraph{Setup} We want to generate labeled data for Interventions in EBM-NLP using gazetteer and we have a small set of expert labeled set for analysis too. Initially, we construct a gazetteer using drug names from RxNorm only. We use similar entity linker as CoNLL and then train the model on the labeled set. 

% The RxNorm only gazetteer will miss the non-pharmaceutical interventions (for example, surgeries and therapies). The goal is -- Can using influence surface these issues?

% \noindent\paragraph{Data} We have 5000 abstracts in train set labeled via gazetteer. The RxNorm gazetteer contains approx. 140K drug names. We also have approx. 160 documents for testing purposes.

% In addition, we derive a corpus of therapies and surgeries from MeSH terminology (approx. 5K items). We add them to gazetteer later on to measure whether it improves the performance of the model in terms of recall.


% \noindent\paragraph{Results} The results are in Table~\ref{tab:ebm_gaz}. We see an more increase in the recall for therapies compared to Drugs but at the cost of precision.
